Learnable and Instance-Robust Predictions for Online Matching, Flows and Load Balancing

We propose a new model for augmenting algorithms with predictions by requiring that they are formally learnable and instance robust. Learnability ensures that predictions can be efficiently constructed from a reasonable amount of past data. Instance robustness ensures that the prediction is robust to modest changes in the problem input, where the measure of the change may be problem specific. Instance robustness insists on a smooth degradation in performance as a function of the change. Ideally, the performance is never worse than worst-case bounds. This also allows predictions to be objectively compared. We design online algorithms with predictions for a network flow allocation problem and restricted assignment makespan minimization. For both problems, two key properties are established: high quality predictions can be learned from a small sample of prior instances and these predictions are robust to errors that smoothly degrade as the underlying problem instance changes.

==> intro.tex <==
	
\section{Introduction}



There is a growing interest in augmenting algorithms with predictions, especially in online algorithm design~\citep{DBLP:journals/siamcomp/GuptaR17,DBLP:conf/icml/BalcanDSV18,DBLP:conf/nips/BalcanDW18,ChawlaGTTZ19,Kraska,MLCachingLykouris,PurohitNIPS,DBLP:conf/soda/LattanziLMV20}. Algorithms augmented with predictions have had major empirical success in domains such as look-up tables~\cite{Kraska}, caching \cite{MLCachingLykouris} and bloom-filters~\cite{Mitzenmacher}.    

These empirical successes have motivated the development of a new model to theoretically analyze algorithms with predictions, with the goal of going beyond worst-case lower bounds in the presence of accurate predictions.  In the  model, an algorithm is given access to a prediction about the problem instance.  The performance of the algorithm is bounded in terms of the error of this prediction.  For example, the competitive ratio or running time can be parameterized by the prediction error.   See \cite{MitzenmacherVassilvitskii} for a survey. 

% changing to plural "models" here is confusing, previous paragraph alludes to one model
Typically in considered models, an algorithm is given access to an \emph{error prone} prediction.  This prediction can be leveraged to make algorithmic decisions.  Ideally, (1) useful predictions result in better performance than the best worst-case lower bound and (2) the algorithm never performs asymptotically worse than the best worst-case algorithm even if the prediction error is large, (3) inbetween there is a graceful degradation in performance as the error in the prediction becomes worse.

This model is a widely applicable framework for beyond-worst-case analysis.  Still, our understanding of this model is in its infancy.  There is a need to refine this model to ensure predictions can be formally learned 
%and the model should provide improved ways to measure the error in the predictions. 
and there is room to explore new and potentially better ways to measure prediction error.

This paper presents a new refinement of the algorithms augmented with predictions model.

\medskip
\noindent \textbf{Learnable and Distributional Robust Predictions:}  This paper provides a new model with two new aspects, learnability and distributional robustness. In its entirety, the model proposed in this paper has three pillars for augmenting algorithms with predictions: (1: \textbf{Existence}) showing the existence of good predictions an algorithm can use to go beyond worst-case lower bounds. Moreover, the predictions should be generalizable and be shown to work well for distributions of problem instances. (2:  \textbf{Robustness}) ensuring predictions are robust to minor changes in the problem instance and (3: \textbf{Learnability}) proving the ability to learn the predictions from representative data.  Our new model incorporates learnability in the predictions for the first time.  Moreover, the model suggests a different way to measure robustness then considered in prior work.

\tl{What are the parentheses for in the next two paragraphs?}

(Learnability) Building on developments in the related area of data driven algorithm design~\citep{DBLP:journals/siamcomp/GuptaR17}, this paper asserts that predicted parameters should be provably learnable and have small sample complexity in the unknown distribution model.  Sample complexity can be used to compare how easy or hard different predictions are to construct. Additionally, ensuring learnability rules out unreasonable predictions.



% Like the  further desire that the algorithms performance degrades as a function of the error in the prediction. In particular, we desire  an algorithm to be robust to inconsequential changes in the input.  Moreover, the framework should allow for comparison of the robustness of different algorithms.  

(Robustness) The new model incorporate aspects of distributionally robust optimization for measuring the degradation in performances as a function of the error in the prediction. Assume the prediction is good for a distribution $\cD$ (e.g. has small competitive ratio).  With this prediction, say the algorithm is run on a problem instance drawn for a different unknown distribution $\cD'$. The expected performance of the algorithm is bounded as a function of the difference in the two distributions. This robustness definition has the added benefit of allowing one to compare the usefulness of different predictions applied to the same problem; an issue not addressed in current models \cite{MitzenmacherVassilvitskii}. 

Learnability and robustness give a natural tradeoff. Some parameters that are easy to learn will not be robust and others that are more difficult to learn can be more robust.



We consider two online problems in this new model.

\medskip \noindent \textbf{Matchings and Flows:} We consider a general flow and matching problem.   As input, we are given a Directed-Acyclic-Graph (DAG) $G$. Each node $v$  has an associated capacity $C_v$.  Moreover we have a special sink node $t$, such that all nodes in the DAG can reach the sink.
For the development of our results, it is instructive to consider layered DAGs where all arcs go from one layer to the next, where the layers are defined by the longest path to the sink (or from a dummy source node connected to all the sources).
	
Online source nodes arrive that have no incoming edges (and  never have any incoming edges in the future) and the other nodes are offline and fixed.  We will refer to online nodes $I$ as impressions.  When impression $i$ arrives, it is connected to a subset of nodes $N_i$.  At arrival, the algorithm must decide a (fractional) flow from $i$ to $t$ of value at most 1 obeying the node capacities.  This flow is fixed the moment the node arrives.  The goal is to maximize the total flow that reaches $t$ without exceeding node capacities.

This problem captures fractional versions of combinatorial problems such as online matching, Adwords, and finding a maximum independent set in a laminar matroid or gammoid.  We call the problem the Online Flow Allocation Problem.

\medskip \noindent \textbf{Restricted Assignment Makespan Minimization:}. We consider the problem of minimizing makespan in the restricted assignment setting.  In this problem, there are $m$ machines and $n$ jobs arrive in an online list.  When job $j$ arrives it must be immediately and irrevocably assigned to a machine.  The job has size $p_j$ and can only be assigned to a subset of machines specific to that job.  After $j$ is assigned the next job arrives.  The goal is to minimize the makespan of the assignment. 


%This  theoretical model holds the promise of giving a systematic approach for going beyond-worst-case analysis.  While exciting, results shown in the model need to be carefully considered as the model can be abused.   Models developed so far are critically missing formal approaches for establishing which predictions are reasonable, the ability to formally compare different measures of prediction error.

%This paper presents a refinement of the algorithms augmented with predictions model designed to overcome these shortcomings.   
%We consider a general class of flow allocation problems and load balancing in the restricted assignment settings where fractional assignments are allowed. Te flow allocation problem captures unweighted bipartite matching   Building on the work of \cite{LattanziLMV20} we establish that there is a vector of weights $\beta$ that can be predicted.  There is one weight per node in the flow problem or one weight per machine in the scheduling problem.  

%\medskip \noindent \textbf{Open Questions:} The algorithms augmented with predictions model has revealed there is a broad potential to circumvent worst-case lower bounds, especially in the online setting using predictions.  The new question is that now that we have restricted ourselves to predictions that are learnable and distributionally robust, can we achieve similar results?



\subsection{Results for Example Problems}


The paper shows that there exists predictions that can be efficiently learned and are distributional robust for both applications.   We show the following theorem regarding matchings and flows.   These predictions break through worst-case lower bounds as a $1-\frac{1}{e}$ lower bound is known on any randomized algorithm for online fractional matching.  Moreover, for integral flows we show a $\Omega(\frac{1}{d})$ lower bound on any deterministic online algorithm for the case of a $d$-layer graph. 

\begin{theorem}[Informal]
There exists predictions for the Online Flow Allocation problem that are:
\begin{itemize}
\itemsep0em 
\item (Existence) Give near a optimal solutions for a single problem instance and generalize to distributions.
\item (Learnable) Are polynomial sample complexity
\item (Robustness) The predictions are distributionally robust.
\end{itemize}
\end{theorem}

For the restricted assignment problem existence predictions was shown in \citep{DBLP:conf/soda/LattanziLMV20}. We remark that the paper leaves open the question if there predictions have small sample complexity or can be formally leaned in any model.   Moreover, it is not known if they are distributionally robust.\footnote{The paper does show another kind of robustness, which refer to as parameter robustness.  See Section~\ref{sec:model} for a comparison.}. We show that the predictions of \citep{DBLP:conf/soda/LattanziLMV20} have much stronger properties than what is known. They are indeed learnable and distributional robust. 

\begin{theorem}[Informal]
There exists predictions for the Restricted Assignment Makespan Minimization problem that are:
\begin{itemize}
\itemsep0em 
\item (Existence) Give near a optimal solutions for a single problem instance when jobs can be assigned \emph{fractionally} and this generalizes to distributions.
\item (Learnable) Are polynomial sample complexity
\item (Robustness) The predictions are distributionally robust.
\end{itemize}
\end{theorem}

We remark this this theorem assumes fractional assignments.  \citep{DBLP:conf/soda/LattanziLMV20} shows that any fractional assignment can be rounded online loosing a $O((\log \log m)^3)$ factor in the makespan.  There is a $\Omega(\log m)$ lower bound on any online algorithm. Together this results in a better than worst case algorithm.  

\smallskip 
\noindent \textbf{Existence:}  Consider the flow allocation problem.   This paper  establishes that there is a single weight that can be predicted for each node in the DAG to route the flows near optimally. These weights are in the same spirit as weights used in other works on Adwords~\citep{PropMatchAgrawal} and scheduling~\citep{DBLP:conf/soda/LattanziLMV20}.  The weights can be used to allocate flow for each impression such that the flow for each impression is deterministic and computed independently of other impressions.
This flow is routed by splitting the ongoing flow to the sink in a proportional manner based on the weights of a node's descendants and their distances from a dummy source connected to all the source nodes (generalizing their layer number). Moreover, the flow is near optimal. Because the flow can be computed in one forward pass for each impression in isolation, they naturally can be used online. These weights are also efficiently computable offline given the entire problem instance.

The predictions for the flow allocation problem and the predictions of \citep{DBLP:conf/soda/LattanziLMV20} are shown to generalize to distributions.  This is immediately implied by the robustness results discussed below when there is no change in the two distributions. 





\smallskip 

\noindent \textbf{Learnability:}  We show that the weights have low sample complexity for both problem.  Consequently, if there is an unknown arbitrary distribution that the impressions or jobs are drawn from, then only a small number of instances is required to compute the weights.   For the flow problem, the number of samples is proportional to size of the DAG without the impressions. For the scheduling problem, it is proportional to the number of machines.  In  problems such as Adwords, the impressions are much larger than the fixed portion of the graph. Similarly, when scheduling the number of jobs is typically much larger than the number of machines.



\smallskip \noindent 
\textbf{Robustness:}   We consider the robustness of the predictions over distributions on the types of impressions and jobs for the two problems.  The type of an impression is defined by the subset of $V$ to which it has outgoing arcs or the subset of machines a job can be scheduled on.     We show that if the weights are near optimal for one distribution, the performance for either problem degrades gracefully according to the difference in the two distributions.  

We further show that our predictions have parameter robustness, the kind of robustness that has been considered in some prior work.




\noindent \textbf{Paper Organization:} The paper is organized as follows.
Section~\ref{sec:relatedwork} surveys related work.  Section~\ref{sec:model} introduces the model. The main results and a high level overview of the analysis is given first and the technical analysis appears next.  \textcolor{red}{\textbf{BEN: WE NEED TO FILL THIS OUT}}


\input{related}

\section{Algorithms Augmented with Learnable and Distributionally Robust Predictions}
\label{sec:model}

In this section, we formalize our model.  The model has three aspects: existence, learnability, and robustness.  The key aspects of the model are the following:




\medskip \noindent \textbf{Existence:}  Consider any  online or offline problem. Let $I$ be the input instance.  The first step is to show the existence of a prediction for any instance $I$.  The algorithm is given a prediction $\hat{y}(I)$ as input along with $I$.  $\hat{y}(I)$ is part of the initial input and $I$ may arrive online.     $\hat{y}(I)$ is a polynomially sized vector.  The prediction  $\hat{y}(I)$ can be used to make algorithmic decisions.  

Next we require that a prediction generalizes.  That is, given a distribution over problem instances $\cD$ it is the case that there is a prediction  $\hat{y}(\cD)$ that an algorithm can use to get strong expected performance on an instance drawn from $\cD$.

A prediction is said to be \emph{useful} if it allows the algorithm to perform better than worst-case lower bounds when  $\hat{y}(I)$ is exact and error-free.  Similarly,  given an error free $\hat{y}(\cD)$ an algorithm should have expected performance better than the best worst-case algorithm for a problem instance drawn from $\cD$. Ideally, the prediction is useful.


\medskip \noindent \textbf{Learnability via Sample Complexity:} We desire that  $\hat{y}(\cD)$ is learnable.  The learnability is an entirely offline problem even if the problem considered is online. Fix a problem and a prediction $\hat{y}()$ for the problem.   There is an \emph{unknown} distribution $\cD$ over problem instances. The question is how many samples are $\cD$ are required to learn the  $\hat{y}(\cD)$ that results in the best performance if $I$ is drawn from $\cD$.   The higher the accuracy and the smaller the sample complexity, the better.    We require the sample complexity to be polynommial in the problem size to qualify as being efficiently learnable in our model.  Note  that it is possible that some predictions could have sublinear sample complexity.
 

\medskip \noindent \textbf{Distributional Robustness:}   Let $\cD'$ and $\cD$ be two distributions over problem instances. Say that  $\hat{y}(\cD)$ results in an algorithm $A(\hat{y}(\cD),I)$ having good performance if $I$ is drawn from  $\cD$.     Then say that $\hat{y}(\cD))$ is used from a problem instance $I'$ drawn from a similar distribution $\cD'$.  Intuitively, $\cD'$ is an  incorrect distribution similar to the real distribution $\cD$. The expected performance of the algorithm should be bounded as a function of the difference between the two distributions.   The distributions considered are not defined a priori, but are problem dependent.   Moreover, it is desirable if the algorithm never performs worst than the best worst case algorithm. 

For instance, say $\hat{y}(\cD)$ can be used to give  a  $c$-competitive algorithm in expectation if the instance is drawn from $\cD$. A result could be the algorithm is $\min\{c\gamma, \alpha\}$-competitive where $\cD$ and $\cD$' differ by a $\gamma$  factor in the $\ell_1$ norm and $\alpha$ is the competitive ratio in the worst case model. 

We remark that the online model still requires $I'$ to be online.  In particular, the arrival order of the sampled instance $I'$   is still online and arrives in worst-case order. 

\medskip \noindent \textbf{Putting it Together:} In summary, the main requirements fo the model are.
\begin{itemize}
\item There should exists a prediction $\hat{y}(I)$ that results in an algorithm having strong performance when given the prediction at the beginning. Ideally, the prediction should  result in a better than worst-case algorithm for any instance $I$.
\item The prediction should generalize to a class of distributions $\cD$. In particular, there should be a prediction $\hat{y}(\cD)$ that results in a better than worst-case algorithm for any instance $I$.  This should hold even if $I$ arrives in worst case order. 
\item The prediction $\hat{y}(\cD)$ should be learnable to sufficiently high accuracy with polynomial sample complexity.
\item Let $\cD'$ and $\cD$ be two distributions over problem instances. Say $\hat{y}(\cD)$ is the generalized prediction for the distribution $\cD$  and $A(\hat{y}(\cD),I)$ has strong performance if $I$ is drawn from $\cD$.  If $I$ is drawn from $\cD'$ then the algorithm's performance should degrade slowly as a function of the difference in the distributions $\cD$ and $\cD'$.  Ideally, even if the distributions are very different the algorithm never has performance worse than the best worst case algorithm.
\end{itemize}
%The advantage of this new model for measuring robustness critically allows for the objective comparison of different predictions.   That is, one can compare how robust two predictions are to the same change in the distribution. This is not true of all error models being considered by the community, as discussed below. 


%Consider a distribution $\cD$ over problem instances.   Let $\cD'$ be a different distribution over instances where the CDF differs from $\cD$  by a parameter $\eps$. Say an algorithm is given a prediction learned on $\cD'$, the error prone distribution.  Then if the prediction is used on a new instances drawn from the similar distribution $\cD'$ then the algorithm should have performance bounded by a function of $\eps$. 

%This new way to measure robustness measures algorithmic performances as a function of the error in the expected instance. We call this distributional robustness. This mseasure transcends the prediction used and gives a concrete way to compare the use of different predictions.

\subsection{Putting the Model in Context}

We now put the model in context. 

\medskip \noindent \textbf{Relationship to Prior Predictions Model:} Existence is effectively the same between our model and that considered in recent work \cite{MLCachingLykouris,PurohitNIPS,ACEPS20}.    All of these results give algorithms that have competitive ratios better than worst-case algorithms when the predictions are error-free. 



The first main difference is how error is measured.   The performance of the algorithm is bounded in terms of the error in the prediction in the prior model.  For example, say the algorithm is given a predicted vector $\hat{y}(I)$ for problem instance $I$ and the true vector that should have been predicted is $y^*(I)$. Let $\eta_{\hat{y}(I)} = \|\hat{y}(I) - y^*(I) \|_p$ be the \emph{error} in the parameter for some norm $p\geq 1$.  The goal is to give an algorithm that is $f(\eta_{\hat{y}(I)})$-competitive for an online algorithm where $f$ is some function of $\eta_{\hat{y}(I)}$.    One could also consider run time or approximation ratio similarly. Notice the bound is worst-case for a given error in the prediction. This we call \emph{parameter robustness}. 

There are two shortcomings with the model.  This first is robustness. Great care has been taken in prior work to ensure an algorithm has strong parameter robustness.  However, parameter robustness has several shortcomings as compared to distributional robustness. 
  The issue is that the error is relative to a parameter, not a uniform baseline and is not scale invariant.  For instance  say an algorithm $A$ is $\eta_{\hat{y}}$-competitive using the prediction $\hat{y}(I)$ and $p=1$.  Now consider a different predicted parameter $\hat{z}(I)$ and set  $\eta_z := \|\hat{z}(I) - z^*(I) \|_1$.  We can make an algorithm $B$ that is $\frac{1}{c} \eta_{z(I)}$-competitive for any $c$.  All we have to do is set $z(I) := \frac{1}{c}y(I)$ and $z^*= \frac{1}{c}y^*(I)$.
  
  This scale invariance makes it difficult to compare the performance of two different predictions.  Moreover, it us unclear how parameter robustness relates to the change in a problem instance.  We fix this with distributional robustness  in model with propose. Distributional robustness allows for easy comparison of two predictions and directly incorporates that a prediction is robust to modest changes in the input.



The next  is \emph{learnability}.  With the notable exception of \cite{DBLP:conf/icalp/JiangP020},  the prior work on this model has introduced predictions without establishing they are learnable.  Without this requirement there is no objective metric to detail if a prediction is reasonable or not.  To see this shortcoming, imagine simply predicting the optimal solution for the problem instance.  This is  often not a reasonable prediction because the optimal solution is too complex to learn and use as a prediction.  We introduce  bounded sample complexity for learning predictions in our model to ensure predictions can be provably learned and unreasonable predictions are ruled out.

     
 % For example, it is not obvious now to compare the competitive of two different algorithms using different predictions.  Say an algorithm $A$ is $\eta_y$-competitive using the prediction $\hat{y}$ and $p=1$.  Now consider a different predicted parameter $\hat{z}$.  We set $z^* =  c y^*$ and $\hat{z} = c\hat{y}$ for arbitrary $c \geq 1$.   Consider an algorithm $B$ that is given $\hat{z}$, uses this prediction to construct  $\hat{y}$, and runs $A$ using $\hat{y}$.   Observe that competitive ratio of $B$ looks much stronger than $A$'s competitive ratio.  Indeed, $\eta_z := \|\hat{z} - z^* \|_1 = c \| (\hat{y} - y^*) \|_1 = c \eta_y $. Now by definition, $B$ is $\eta_y$-competitive.  However, $\eta_y = \frac{1}{c} \eta_z$.  Thus the algorithm is $\frac{1}{c} \eta_z$-competitive.  On the surface, it would seem $B$ is much stronger than $A$.



\medskip \noindent \textbf{Learning Algorithm Parameters:}  In our model, one is showing how to learn parameters for an algorithm.  The model is simultaneously grounded in stochastic analysis for learnability and robustness. Given this, a question one may ask is why not simply learn the input distribution and then use a stochastic analysis.   

Learning algorithmic parameters has distinct advantages over learning a distribution.  This advantage is why the model has the potential to reveal interesting new algorithmic insights into  problems.  Indeed, in many cases it can be easier to learn a decision rule than it is to learn a distribution. This differentiates the insights that can be gained in the model versus a direct stochastic analysis.    

For example, consider the unweighted $b$-matching problem in bipartite graphs for large $b$ in the online setting.  Nodes on one side of the graph arrive online and must be matched on arrival.  Say the nodes are i.i.d. sampled from an unknown discrete distribution over types. A type is define by the neighbors of the node.  Let $s$ be the number of types. Then the sample complexity of learning the distribution is at least $\Omega(s)$. Notice that $s$ could be superlinear.  However, it is known \cite{XXX} that for this problem, an algorithm can be learned that requires a sublinear number of samples.

The phenomenon that it is easier to learn good algorithmic parameters than the underlying input distribution the algorithm is facing has been observed in several prior works.  See \cite{XXX} for details.

{\color{red} \textbf{Chenyang: Maybe we can explain distributional Robustness in this way:} \color{black} although the distribution is hard to be predicted directly (we need to find some other algorithmic parameters to predict), the distribution provides us a platform to connect different parameters predictions. We can assume that we have a way to predict the distribution of an online instance when comparing different parameter predictions. We compute different algorithmic parameters from the predicted distribution, apply them to a new online instance and bound all their performances by the error of the two instance distributions. In this way, we can compare the competitive ratio of different predictions. Note that some algorithmic parameters may fluctuate sharply even if the distribution of instance changes a little bit. If only checking the parameter robustness, these parameters seem to be good predictions. But in practice, the predicted error of these parameters will always be very large since they are very sensitive. }

\medskip \noindent \textbf{Relationship to Prior Work:}  To illustrate how the model compares to some prior work, consider some of the papers in this area.  The first column states if they prove the existence of useful predictions.  The second denotes if the error is bounded in terms of error in the predicted parameter.  The third and fourth denotes whether they are robustness with respect to the parameter or distribution. Finally, the last is if the parameter predicted is provably learnable.  


\begin{center}
\begin{tabular}{p{130pt}p{70pt}p{70pt}p{70pt}p{70pt}}%{ l c c c c }
 Problem & Existence & Parameter \quad Robustness & Learnability & Distributional Robustness \\ 
\hline

 Caching & \cite{MLCachingLykouris,DBLP:conf/soda/Rohatgi20,DBLP:conf/icalp/JiangP020,WeiCaching20} & \cite{MLCachingLykouris,DBLP:conf/soda/Rohatgi20,DBLP:conf/icalp/JiangP020,WeiCaching20} & - & -\\
 Completion~Time~Scheduling & \cite{PurohitNIPS} & \cite{PurohitNIPS} & - & -\\    
 Ski Rental & \cite{PurohitNIPS,anand2020customizing,DBLP:conf/icml/GollapudiP19} & \cite{PurohitNIPS,anand2020customizing,DBLP:conf/icml/GollapudiP19} & \cite{anand2020customizing}& - \\
 \hline
 Restricted Assignment & \cite{DBLP:conf/soda/LattanziLMV20} & \cite{DBLP:conf/soda/LattanziLMV20} &   This Paper  & This Paper \\
   Adwords &\cite{PropMatchAgrawal} &  This Paper  & This Paper & This Paper \\  
 Flows &  This Paper  &  This Paper  &  This Paper &  This Paper 
 \end{tabular}
\end{center}

{\color{red} \textbf{Chenyang: is ``Adwords" ok here? Or maybe we say ``matching"?}}

Extending this line of literature, we show there exists predictions that have all four properties simultaneously. 



%The direct approach is to learn the unknown distribution from samples and utilize known ideas from stochastic optimization (where knowledge of the distribution is key). However, if the number of item types (denoted by s) is very large, the sample complexity for learning the distribution could be huge. However, if we only aim to learn the threshold ϴ, the sample complexity becomes much smaller. More precisely, the pseudo-dimension of this threshold is at most log(s). Also, from previous work (Rishi Gupta & Tim Roughgarden, 2017), the sample complexity is O(log(s)) which is significantly smaller. 




==> oldtext.tex <==
\section{Introduction}



Inspired by advances in machine learning, there is a growing interest in augmenting algorithms with predictions, especially in online algorithm design~\cite{DBLP:journals/siamcomp/GuptaR17,DBLP:conf/icml/BalcanDSV18,DBLP:conf/nips/BalcanDW18,ChawlaGTTZ19,Kraska,MLCachingLykouris,PurohitNIPS,DBLP:conf/soda/LattanziLMV20}. Algorithms augmented with predictions have had major empirical success in domains such as look-up tables~\cite{Kraska}, caching \cite{MLCachingLykouris} and bloom-filters~\cite{Mitzenmacher}.
%\ravi{These successes and the availability of predictions motivate the development of a possibility of a new model that goes beyond worst-case bounds when supplied with accurate predictions.}
These successes and the availability of data to make predictions using machine learning have motivated the development of new analysis models for going beyond worst-case bounds where an algorithm is supplied with accurate predictions.
%These empirical successes have motivated the development of a new model to theoretically analyze algorithms with predictions, with the goal of going beyond worst-case bounds in the presence of accurate predictions.  
In the  model, an algorithm is given access to a prediction about the problem instance.  
The performance of the algorithm is bounded in terms of the quality of this prediction.
%Typically in such a model, an algorithm is given access to an \emph{error prone} prediction.  This prediction can be leveraged to make algorithmic decisions.   Ideally, (1) the predictions result in better performance than the best worst-case bound.  We say such predictions are \emph{useful}; (2) the algorithm never performs asymptotically worse than the best worst-case algorithm even if the prediction error is large; and (3) in-between,  there is a graceful degradation in performance as the error in the prediction becomes worse. For example, the competitive ratio or running time can be parameterized by the prediction error.   See \cite{MitzenmacherVassilvitskii} for a survey.
Typically the algorithm learns such predictions from a limited amount of past data leading to  \emph{error-prone} predictions.
%thatcan be leveraged to make decisions. 
The algorithm with accurate predictions should result in better performance than the best worst-case bound. Ideally, the algorithm never performs asymptotically worse than the best worst-case algorithm even if the prediction error is large.  In-between,  there is a graceful degradation in performance as the prediction error increases. For example, competitive ratio or running time can be parameterized by prediction error. See \cite{MitzenmacherVassilvitskii} for a survey.
% changing to plural "models" here is confusing, previous paragraph alludes to one model


%This model is a widely applicable framework for beyond-worst-case analysis.  Still, our understanding of this model is in its infancy.  There is a need to refine this model to ensure predictions can be formally learned and there is room to explore new and potentially better ways to measure prediction error.
%This paper presents a new refinement of the algorithms augmented with predictions model.

\subparagraph*{Learnable and Instance Robust Predictions:}  The model proposed in this paper has two pillars for augmenting algorithms with predictions. (\textbf{Learnability}:) Predictions should be learnable from representative data.  (\textbf{Instance Robustness}\footnote{Note that the robustness here is different from the definition of robustness mentioned in previous work, which we refer to as parameter robustness. 
See Section~\ref{sec:model} for a discussion.
%A further discussion is deferred to Section~\ref{sec:model}.
} :) Predictions should be robust to minor changes in the problem instance. 

Suppose  there is an unknown distribution $\cD$ over instances $\cI$.  Building on  data driven algorithm design~\cite{DBLP:journals/siamcomp/GuptaR17} and PAC-learning models, we require that predicted parameters are provably learnable  using a small number of sample instances from $\cD$.  The sample complexity of this task can be used to compare how difficult different predictions are to construct.  Practically, the motivation is that parameters are learned from  prior data (e.g.  instances of the problem). 

%In practice, future problem instances may not come from the distribution $\cD$ the parameters are learned from. 
%\tl{In practice, future problem instances may not come from the same distribution used to learn the parameters.}
Therefore, we also desire predictions that are robust to modest changes in the input. 
In particular, if the predictions perform well on some instance $\cI$, then the performance on a nearby instance $\cI'$ should be bounded as a function of the difference between these instances.  
%Instance robustness is a natural definition that has the benefit of allowing one to compare the usefulness of different predictions applied to the same problem  \cite{MitzenmacherVassilvitskii}.
%\ravi{Maybe add a sentence here about how instance robustness is better than parameter robustness, or delete the last sentence and address later.}

% if the performance of the algorithm using the prediction $\hat{y}(\cI)$ on the instance $\cI'$ can be bounded as a function of the difference between these two instances.

%In contrast, prior work focuses on bounding the degradation in algorithm performance as a function of the difference in the predicted parameter  $\hat{y}$ and the optimal prediction $y^*(\cI)$ for the same instance $\cI$ (we call such predictions {\em parameter robust}).\footnote{$\hat{y}$ in this model can be arbitrary and is not instance dependent.}



% Like the  further desire that the algorithms performance degrades as a function of the error in the prediction. In particular, we desire  an algorithm to be robust to inconsequential changes in the input.  Moreover, the framework should allow for comparison of the robustness of different algorithms.

% The performance of any algorithm given the predictions should degrade gracefully as a function of the changes in the input.
%The new model incorporate aspects of distributionally robust optimization for measuring the degradation in performances as a function of the error in the prediction. Assume the prediction is good for a distribution $\cD$ (e.g. has small competitive ratio).  With this prediction, say the algorithm is run on a problem instance drawn for a different unknown distribution $\cD'$. The expected performance of the algorithm is bounded as a function of the difference in the two distributions.

%\tl{Please read above paragraph carefully, do we need to explain more about parameters here for context?}
%\rr{This may be a bit early for this, but we could add a sentence preempting the distribution or type robustness coming later here.}

%Learnability and robustness give a natural tradeoff. Some parameters that are easy to learn will not be robust while others that are more difficult to learn can be more robust. 
We note that learnability is rarely addressed in prior work and our robustness model differs from many prior works by bounding the error by differences in problem instances (instance robustness), rather than by the differences in the predictions themselves (parameter robustness).
We present learnable and instance-robust predictions for two concrete online problems.
%Next, we consider two concrete online problems in this new model to demonstrate what can be achieved under it.

%\smallskip
%\noindent \textbf
\subparagraph*{Online Flow Allocation Problem:} We consider a general flow and matching problem.   The input is a Directed-Acyclic-Graph (DAG) $G$. Each node $v$  has an associated capacity $C_v$.  There is a sink node $t$, such that all nodes in the DAG can reach the sink.
%For the development of our results, it is instructive to consider layered DAGs where all arcs go from one layer to the next, where the layers are defined by the longest path to the sink (or from a dummy source node connected to all the sources).
Online source nodes arrive that have no incoming edges (and  never have any incoming edges in the future) and the other nodes are offline and fixed.  We will refer to online nodes $I$ as impressions.  When impression $i$ arrives, it is connected to a subset of nodes $N_i$.  At arrival, the algorithm must decide a (fractional) flow from $i$ to $t$ of value at most 1 obeying the node capacities.  This flow is fixed the moment the node arrives.  The goal is to maximize the total flow that reaches $t$ without exceeding node capacities.

This problem captures fractional versions of combinatorial problems such as online matching, unweighted Adwords, and finding a maximum independent set in a laminar matroid or gammoid.  We call the problem the Online Flow Allocation Problem.

%\smallskip
%\noindent\textbf
\subparagraph*{Restricted Assignment Makespan Minimization:} In this problem, there are $m$ machines and $n$ jobs arrive in an online order.  When job $j$ arrives it must be immediately and irrevocably assigned to a machine.  The job has size $p_j$ and can only be assigned to a subset of machines specific to that job.  After $j$ is assigned the next job arrives.  The goal is to minimize the makespan of the assignment. 


%This  theoretical model holds the promise of giving a systematic approach for going beyond-worst-case analysis.  While exciting, results shown in the model need to be carefully considered as the model can be abused.   Models developed so far are critically missing formal approaches for establishing which predictions are reasonable, the ability to formally compare different measures of prediction error.

%This paper presents a refinement of the algorithms augmented with predictions model designed to overcome these shortcomings.
%We consider a general class of flow allocation problems and load balancing in the restricted assignment settings where fractional assignments are allowed. Te flow allocation problem captures unweighted bipartite matching   Building on the work of \cite{LattanziLMV20} we establish that there is a vector of weights $\beta$ that can be predicted.  There is one weight per node in the flow problem or one weight per machine in the scheduling problem.

%\medskip \noindent \textbf{Open Questions:} The algorithms augmented with predictions model has revealed there is a broad potential to circumvent worst-case lower bounds, especially in the online setting using predictions.  The new question is that now that we have restricted ourselves to predictions that are learnable and distributionally robust, can we achieve similar results?


\subsection{Overview of Results for Flow Allocation and Restricted Assignment}

This paper shows that there are %predictions 
algorithmic parameters
that can be efficiently learned and are instance robust for both applications. \xcy{We now introduce main results for the two problems.}
%These predictions are useful and give better than worst-case bounds.
%We show the following theorem regarding online flow allocation.  
%The predictions break through worst-case bounds as a $1-\frac{1}{e}$ bound is known on any randomized algorithm for online fractional matching that the problem generalizes.  Moreover, for integral flows we show a $1/(d+1)$ bound on any deterministic online algorithm for the case of a $d$-layer graph.
For the online flow allocation problem,
we  predict a single weight for each node of the DAG. These weights are learnable and only a small number of samples are required to construct weights that are near optimal. 
These predictions break the worst-case $1-\frac{1}{e}$ bound on the competitive ratio for any randomized algorithm for online fractional matching\tl{, a special case.} 
\xcy{Moreover, we define a reasonable distance measure between instances and show that the optimal parameters of an instance have a competitive performance on its nearby instances, which is referred to ``Instance Robustness''. Besides,}
%that the problem generalizes.  
%Moreover, the ratio is never worse than the $1/(d+1)$ bound that we prove that any deterministic integral online algorithm cannot beat (Theorem~\ref{thm:worst_case_bound}) for the case of a $d$-layer graph.
\tl{the ratio is never worse than $\frac{1}{d+1}$, which is tight for deterministic integral online algorithms and $d$-layer graphs (see Theorem~\ref{thm:worst_case_bound})}.
\begin{theorem}[Flow Allocation - Informal]
There exist algorithmic parameters for the Online Flow Allocation problem with the following properties:
%\begin{itemize}
%\itemsep0em
\begin{enumerate}[(i)]
%\item \ben{(Beyond Worst-Case Bounds) Optimal parameters can be used by an algorithm to give a $(1-\eps)$-approximation for any  constant $\eps >0$. 
\item (Learnability) Learning near-optimal parameters has  sample complexity polynomial in $\frac{1}{\epsilon}$ and the size of the graph  excluding the impressions. These parameters result in an online algorithm that is a  $(1-\eps)$-approximate solution in expectation as compared to the expected optimal value on the distribution  for any  constant $\eps >0$. (Theorem~\ref{thm:DAG-learnability})
\item (Instance Robustness) \tl{There exists a metric such that} using the optimal parameters for any instance on a nearby instance gives a competitive ratio that improves as their distance (w.r.t. the metric) decreases. 
%and never worse than $\frac{1}{d+1}$ no matter how different the instances are for a $d$-layer graph. 
(Theorem~\ref{thm:dist_robustness})
\tl{\item (Worst-Case Robustness) The competitive ratio of the online algorithm using the parameters is never worse than $\frac{1}{d+1}$, regardless of the distance between the two instances. (Theorem~\ref{thm:dist_robustness})}
%%Predicting the parameters gives an instance-robust algorithm, whose competitive ratio is bounded by the difference of the two instances and never worse than $\frac{1}{d+1}$ no matter how different the instances are for a $d$-layer graph.
%The predictions are instance robust and the objective is never smaller than a  $\frac{1}{d+1}$ of optimal no matter how inaccurate the error is for a $d$-layer graph. (Theorem~\ref{thm:dist_robustness}) 
%whose competitive ratio gives a  never worse than $\frac{1}{d+1}$ no matter how inaccurate the error is for a $d$-layer graph.
%Predicting the parameters gives an instance-robust algorithm, whose competitive ratio is bounded by the difference of the two instances and never worse than $\frac{1}{d+1}$ no matter how different the instances are for a $d$-layer graph.
%(Theorem~\ref{thm:dist_robustness})
%\end{itemize}
\end{enumerate}
\end{theorem}

%\textbf{Ben: Check next paragraph carefully!}
%This theorem shows that predictions can be efficiently learned from prior data on a problem. Moreover, the learnability establishes that the learned parameters will give near-optimal performance in expectation if the online instance is drawn from the same distribution. Robustness gives the additional guarantee that the predictions will have robust performance95even if the online instance is adversarial up to modest changes in the instance.
%This theorem shows that there exists algorithmic parameters for online flow allocation that can be efficiently learned from prior data.
%can be efficiently learned from prior data on a problem.  
%Under some mild assumptions (see Theorem~\ref{thm:DAG-learnability}), the learnability establishes that the predictions will give \emph{near optimal performance} in expectation if the online instance is drawn from the same distribution, going beyond the worst-case. 
%Robustness gives the additional guarantee that the predictions 
%will perform well
%will have near-optimal performance 
%on nearby instances %(see Theorem~\ref{thm:dist_robustness})
%even if they are adversarial 
%and never performs worse than the best ratio of a deterministic integral algorithm on an arbitrary instance.

%\smallskip
%\noindent \textbf
\subparagraph*{Node Parameters:} Our results on learnability and robustness are enabled by showing the existence of node weights which capture interesting combinatorial properties of flows.  We establish that there is a single weight 
%that can be predicted 
for each node in the DAG that completely describe near optimal flows on a single problem instance.  These weights are in the same spirit as weights used in other works on Adwords~\cite{PropMatchAgrawal} and scheduling~\cite{DBLP:conf/soda/LattanziLMV20}.  
%The weights can be used to allocate flow for each impression such that the flow for each impression is deterministic and computed independently of other impressions.
The weights determine an allocation of flow for each impression which is independent of the other impressions.
%This flow is routed by splitting the ongoing flow to the sink in a proportional manner based on the weights of a node's descendants and their distances from a dummy source connected to all the source nodes (generalizing their layer number).
Each node in the DAG routes the flow leaving it proportionally to the weights of its outgoing neighbors.
Moreover, the flow is near optimal, giving a $(1-\eps)$-approximate solution for any constant $\eps >0$ (but requiring time polynomial in $1/\epsilon$ to compute). Given these weights, the flow can be computed in one forward pass for each impression in isolation.  Thus they can be used online if given as a prediction. These weights are also efficiently computable offline given the entire problem instance (see Theorem~\ref{thm:weight_existence_3_layer}).
%The existence of node weights as predictions is established in Theorem~\ref{thm:weight_DAG} in Section~\ref{sec:existweight}. As a warm-up, a description of the result for 3-layered DAGs is in Theorem~\ref{thm:weight_existence_3_layer} along with a technical overview in Section~\ref{sec:flows_existence}. 

%\ravi{Given the existence of node weights that are independent of the number of impressions,}
%\smallskip
%\noindent \textbf
\subparagraph*{Learnability:} 

We show that learning near-optimal weights
%weights that give a near  optimal solution in expectation 
has low sample complexity when instances are drawn from an appropriately defined unknown distribution. The number of samples is polynomial in the size of the DAG without the impressions. Note that in problems such as Adwords, the impressions are usually much larger than the fixed portion of the graph. 

%\smallskip
%\noindent \textbf
\subparagraph*{Instance Robustness:}    Instances are defined by the number of each \emph{type} of impression.  The type of an impression is given by the subset of $V$ to which it has outgoing arcs.  We show that if the weights are near optimal for one instance, the performance degrades gracefully according to the difference in the two instances.  We measure the difference of the two instances as the difference of the number of impressions of each type (see Theorem~\ref{thm:dist_robustness}).% in Section~\ref{sec:flows_robustness}. 
%\rr{More generally, we can insist that if there are single set of predictions for a class of distributions over the instances, then the same predictions will perform reasonably well on instances from a nearby distribution. We call such types of robustness requirements as ``instance robustness".}
\footnote{We also show that our predictions for the online flow allocation problem have ``parameter robustness", the kind of robustness that has been considered in prior work (Theorem~\ref{thm:flow_param-rob}).} % Here, the degradation in solution quality is bounded as a function of the relative error from the optimal prediction parameters for the same instance. As an example, \citep{DBLP:conf/soda/LattanziLMV20} study the parameter robustness of predictions for restricted assignment.

%The existence of node weights as predictions is established in Theorem~\ref{thm:weight_DAG} in Section~\ref{sec:existweight}. A description of the result for 3-layered DAGs is in Theorem~\ref{thm:weight_existence_3_layer} along with a technical overview in Section~\ref{sec:flows_existence}. 
%Instance robustness of these weights is shown in Theorem~\ref{thm:dist_robustness} in Section~\ref{sec:flows_robustness}. The learnability is established in Theorem~\ref{thm:DAG-learnability} in Section~\ref{sec:flows_learnability}.


%Next we extend the results to the restricted assignment problem. 

\begin{theorem}[Restricted Assignment - Informal]
There exist algorithmic parameters for the Restricted Assignment Makespan Minimization problem with the following properties:
%\begin{itemize}
%\itemsep0em
\begin{enumerate}[(i)]
    \item (Learnability) Learning the near optimal parameters has  sample complexity polynomial in $m$, the number of machines, and $\frac{1}{\epsilon}$. These parameters result in an online algorithm that is a  $(1+\eps)$ approximate solution in expectation as compared to the expected optimal value on the distribution  for any  constant $\eps >0$. (Theorem~\ref{thm:learnability_makespan})
    \item (Instance Robustness) \tl{There exists a metric such that} using the optimal parameters for any instance on a nearby instance gives a competitive ratio for fractional assignment that is proportional to their distance (w.r.t the metric). 
    %and never worse than $O(\log m)$, matching the known $\Omega(\log m )$ lower-bound on any integral online algorithm.
    %\xcy{By predicting the parameters, the algorithm is instance robust, ensuring the competitive ratio is never larger than $O(\log m)$.
    % factor of optimal. 
    (Theorem~\ref{thm:makespan-robustness})
    %The predictions are instance robust and using them the algorithm 
    \tl{\item (Worst-Case Robustness) The competitive ratio of the algorithm using the parameters is never worse than $O(\log m)$, matching the known $\Omega(\log m )$ lower-bound on any integral online algorithm. (Theorem~\ref{thm:makespan-robustness})}
\end{enumerate}
%\end{itemize}
\end{theorem}

This theorem shows that the predictions of \cite{DBLP:conf/soda/LattanziLMV20} have much stronger properties than what is known and are learnable and instance robust. That paper left open the question if their predictions can be formally learned in any model.   Moreover, it was not known if they are instance robust.  
We remark that this theorem assumes fractional assignments, whereas the original problem (and the lower bound~\cite{OnlineAssignmentsAzar}) requires integer assignments.  Lattanzi et al.~\cite{DBLP:conf/soda/LattanziLMV20} shows that any fractional assignment can be rounded online while losing a $O((\log \log m)^3)$ factor in the makespan.   
%We establish instance robustness in Theorem~\ref{thm:makespan-robustness} and learnability in Theorem~\ref{thm:learnability_makespan}, both in Section~\ref{sec:load_balancing_results}. 



%The predictions for the flow allocation problem and the predictions of \citep{DBLP:conf/soda/LattanziLMV20} are shown to generalize to distributions, represented by their empirically sampled instances.{\color{red} Chenyang: a little bit confused here.}  %This is immediately implied by the robustness results discussed below when there is no change in the two distributions.












%\subparagraph*{Paper Organization:} 
%\smallskip
%\noindent \textbf
\iffalse
\subparagraph*{Paper Organization:}
The paper is organized as follows.
Section~\ref{sec:relatedwork} surveys related work.  Section~\ref{sec:model} introduces the model. The main results and a high-level overview of the analysis is given first and the technical analysis appears next. 
For online flow allocation, Section~\ref{sec:flows_existence}, Section~\ref{sec:flows_robustness} and Section~\ref{sec:flows_learnability}, respectively, corresponds to the technical overviews of the three parts: existence of node predictions, robustness and learnability. All full technical proofs are given in the appendix.
More precisely, for online flow allocation, we show the existence of predictions in 3-layer DAGs in Appendix~\ref{sec:existweight} and give the results for general DAGs in Appendix~\ref{sec:apdxexistweight}.
The proofs about the instance robustness and the parameter robustness are deferred to Appendix~\ref{sec:robustness} and Appendix~\ref{app:robustness} respectively. Finally, we first prove the learnability of predictions in 2-layered graphs in Appendix~\ref{sec:learnability} and then generalize this result to general DAGs in Appendix~\ref{sec:apdxlearnability}.
For load balancing, we present the results in Section~\ref{sec:load_balancing_results} and the corresponding proofs in Appendix~\ref{sec:apdx_scheduling}.
\fi

%\textcolor{red}{\textbf{BEN: WE NEED TO FILL THIS OUT}}


\input{related}



==> results.tex <==

\subsection{Applications: Matchings, Flows, and Load Balancing}




\medskip \noindent \textbf{Matchings and Flows} 

\medskip \noindent \textbf{Load Balancing  in the Restricted Assignment Model}   

We also extend prior work on machine scheduling to show that the predictions considered in \cite{XXX} fall into our model.  The work of \cite{XXX} gave predictions for online scheduling in the restricted assignment setting.  In this model, jobs arrive online and need to be assigned to $m$ machines.  When a job $j$ arrives it can be assigned to a subset of machines $N(j)$.  The job must be irrevocably assigned to a machine on arrival.  The goal is to minimize the makespan, i.e. the maximum total load incurred by jobs on any machine.
	
It is known that there is a $\Omega(\log m)$ lower bound on the competitive ration of any online algorithm and a simple greedy algorithm is $O(\log m)$ competitive.  The work \cite{XXX} showed that accurate predictions can be used to break through this lower bound.  They show a $O(\min \{\log \eta  \log \log^3 m, \log m\})$ competitive algorithm where $\eta$ is the maximum relative error over all predicted parameters. The parameter predicted is a single number per machine, which intuitively represents how one should conserve space on that machine for different job neighborhoods. 
	
This work shows the power for using predictions to go beyond worst case analysis.  One can achieve very small makespan with perfect predictions and the algorithm gracefully degrades to asymptotically match the best worst case algorithm performance with terrible predictions.  However, how can we interpret such results?  Is the number predicted per machine reasonable?  It is unknown if the prediction is learnable. Moreover, as discussed, measuring relative error in a predicted parameter can be misleading.
	
In this work, we complete the picture and show that these parameters are learnable. Moreover, they are  robust over changes in distributions. 
	
%\textbf{Maybe state scheduling results here?  Alternatively we can move the above stuff about scheduling below the matchings and flows and then state the results.}
	

\iffalse

%Our results fulfill the three desiderata for algorithms with predictions for the flow and matching problem. First we establish what to succinctly predict to aid an  algorithm with allocating flows online ({\em existence}).  Second, we show an algorithm using these predictions has robust performance ({\em robustness}).  We demonstrate a prediction that is near optimal with perfect predictions and gracefully degrades in performance as there is larger error in the predictions.  Similar to smooth degradation, we show that if  predictions are constructed with good performance on one known distribution over online arrivals then they will work well on a similar distribution of arrivals. Intuitively, if they are computed from an inaccurate distribution they will still work well if the true distribution is close to it.  Third, we establish that the prediction is efficiently learnable ({\em learnability}).  We show that the predictions can be computed from a small number of instances of the problem for unknown distributions over online arrivals.
	
	\medskip \noindent \textbf{Existence of Predictions:}  We  establish that there is a single weight that can be predicted for each node in the DAG to route the flows near optimally. These weights are in the same spirit as weights used in other works on Adwords~\citep{PropMatchAgrawal} and scheduling~\citep{DBLP:conf/soda/LattanziLMV20}. The weights can be used to allocate flow for each impression such that the flow for each impression is deterministic and computed independently of other impressions.
This flow is routed by splitting the ongoing flow to the sink in a proportional manner based on the weights of a node's descendants and their distances from a dummy source connected to all the source nodes (generalizing their layer number).
%Note in particular that all the flows passing through any node are split in the same proportion irrespective of the originating source.
Moreover, the flow is near optimal. Because the flow can be computed in one forward pass for each impression in isolation, they naturally can be used online. These weights are also efficiently computable offline given the entire problem instance.


Consider a directed acyclic graph $G=(\{s,t\} \cup V, E)$, where each vertex $v\in V$ has capacity $C_v$ and is on some $s-t$ path. Our goal is to maximize the flow sent from $s$ to $t$ without violating vertex capacities (note that there are no edge capacities).
% new text for 3-layer version
Before considering the general version of this problem, we examine the 3-layered version. This case is defined as follows. The vertices in $V$ are partitioned into 3 sets $I,A$, and $B$. $s$ is connected to all of $A$ and $t$ is connected to all of $B$, while the remaining edges are only allowed to cross from $I$ to $A$ and from $A$ to $B$.  Let $N_u := \{v \in V \mid (u,v) \in E\}$ be $u$'s out-neighbors.  We have the following result generalizing the prior work of Agrawal et al~\cite{PropMatchAgrawal}.

% complicated general case, replace w/ 3 layer version in intro
\iffalse
For any vertex $v$, let $d_v$ be the longest distance from $s$ to $v$. Define
$d:=\max_{v\in V\setminus\{t\}}d_v$ and
$d_{uv} := d_v-d_u-1$ for each edge $(u,v)$. We have the following theorem.
	
	\begin{theorem}\label{thm:weight_existence}
		For any edge $(u,v)\in E$, let $x_{uv}$ be the proportion of flow crossing this edge in all flow received by $u$. For any given $\epsilon\in (0,1)$,
		there exists a weight $\alpha_v$ for each vertex $v$ such that we can obtain a $(1-\epsilon)$-approximate solution by setting the proportion of flow out of $u$ to neighbor $v$ to be $ x_{uv} =  \frac{\alpha_v^{1/(2n)^{d_{uv}}}}{ \sum_{v'\in N_u} \alpha_{v'}^{1/(2n)^{d_{uv'}}}  },$
		where $n$ is the number of vertices and $N_u$ is the set of vertices pointed by $u$. Moreover, these weights can be obtained in a time of $O(d^2n^{d+1}\log(n/\epsilon)/\epsilon^2 )$ where $d$ is the diameter of this graph excluding vertex $t$.
	\end{theorem}
\fi

\begin{theorem} \label{thm:weight_existence_3_layer}
	Let $G = (\{s,t\} \cup V, E)$ be a 3-layered DAG.  For each edge $(u,v) \in E$, let $x_{uv}$ be the proportion of flow through $u$ which is routed along $(u,v)$.  For any $\epsilon \in (0,1)$, there exists weights $\{\alpha_v\}_{v\in V}$ such that setting $x_{uv} = \frac{\alpha_v}{\sum_{v' \in N_u} \alpha_{v'}}$ yields a $(1-\epsilon)$-approximate flow. Moreover, these weights can be obtained in time $O(n^3 \log(n/\epsilon) / \epsilon^2)$.
\end{theorem}

We can generalize this theorem to the case of $d$-layered graphs.  In particular, our algorithm for the $d$-layered case produces weights with additional properties, which we leverage to handle general DAGs.  See Section~\ref{YYYYY} for precise statements.


\iffalse
Notice that the number of weights is proportional to the number of nodes in the graph and not the number of edges. Moreover the additional information to compute these flows online ($d_v$) is also linear in the number of nodes.
In the case of layered DAGs, the formula reduces to the proportional flow allocation according to the weights from prior work~\citep{PropMatchAgrawal}.
We believe it is an interesting combinatorial property that such succinct weights on the nodes can encode a good flow on the asymptotically larger number of edges and is of independent interest.
To route a flow from the source, we can use the given weights and the longest distance values on each node and process the nodes in increasing topological order to determine how the total fractional flow arriving at this node should be split and proportionally routed to its descendants.
\fi
% new version of previous paragraph here
Notice that the number of weights is proportional to the number of nodes in the graph and not the number of edges. We believe it is an interesting combinatorial property that such succinct weights on the nodes can encode a good flow on the asymptotically larger number of edges and is of independent interest.


\medskip \noindent \textbf{Learnability of Weights:} Next we show that the weights are efficiently learnable. This helps to clarify why the weights are a natural quantity to predict. Assuming that each arriving impression is i.i.d. sampled from an unknown distribution, we want to learn a set of weights from a collection of past instances and examine their performance on a new instance from the same distribution. 
A direct approach might be to learn the unknown distribution from samples and utilize known ideas from stochastic optimization (where knowledge of the distribution is key). 
A major issue though is that there can be a large number of possible types (potentially exponential in the number of nodes of the DAG).  A distribution that is sparse over types is not easy to learn with a small number of samples.
	
	%Notice that in the above we showed that if the weights are computed on a distribution they are robust to modest modifications of the distribution.  This shows that we can learn a distribution and then compute the weights.  The performances is as good as  how well the distribution fits the impression that arrive online. A major issue though is that there can be a large number of possible types (potentially exponential in the number of nodes of the DAG).  A distribution that  is sparse over types is  not easy to learn with a small number of samples.

We claim that the weights are efficiently learnable, even if the distribution of types of impressions is not. We show that this task has low sample complexity and admits an efficient learning algorithm.  Consequently, if there is an unknown arbitrary distribution that the impressions are drawn from, then only a small number of instances is required to compute the weights. The number of samples is proportional to size of the DAG without the impressions.  In most problems such as Adwords, the number of arriving impressions is much larger than the fixed (offline) portion of the graph.

\begin{theorem}
	Assume that each impression is i.i.d. sampled from an unknown distribution $\D$.
	Let $\cD^m$ be the distribution over length $m$ sequences of impressions in which each entry is an i.i.d sample from $\cD$.
	Under some mild assumptions {\color{red} (Chenyang: a little bit confused about how to mention these assumptions)}, for any $\epsilon,\delta \in (0,1)$, there exists a learning algorithm such that, after observing $O(\frac{n^2}{\epsilon^2}\ln(\frac{n\log n}{\delta}))$ instances,
	it will return a set of weights $\{ \predw \}$, satisfying that with probability at least $1-\delta$,
	$ \E_{I \thicksim \D^m}[R(\predw,I)] \geq (1-\epsilon) \E_{I \thicksim \D^m}[R(\alpha^*,I)]$
	where $R(\alpha,I)$ is the value of the fractional flow obtained by applying $\alpha$ to instance $I$ and $\alpha^* = \arg\max\limits_{\alpha } \E_{I \thicksim \D^m}[ R(\alpha,I) ]$.
\end{theorem}
	


\medskip \noindent \textbf{Robustness of Weights:} Finally, we establish that the predictions are robust to error. Given a set of weights, we bound the performance of the online algorithm in terms of the prediction error.  In particular, we show the performance degrades gracefully in terms of the error. 
As mentioned above, we consider distributional robustness and parameter robustness, giving us two ways of defining error.
	
	%two ways to measure the prediction error.
	
	%We show this in two ways.
To show the distributional robustness, we consider a distribution over types of impressions. The type of an impression is defined by the subset of $V$ to which it has outgoing arcs. 
We show that for a set of weights computed using a type distribution $\cD$, they can be easily transferred to another distribution close to $\cD$. 

%This is a natural quantity to predict from past data, but it is not clear how to use this information to compute allocations online.   

%We show that if the weights are computed using predictions of this type distribution, then	the amount of flow that is lost degrades gracefully according to the error in the distribution predicted.

%The first type of prediction we consider is a distribution over types of impressions.  The type of an impression is defined by the subset of $V$ to which it has outgoing arcs.  This is a natural quantity to predict from past data, but it is not clear how to use this information to compute allocations online.   We show that if the weights are computed using predictions of this type distribution, then	the amount of flow that is lost degrades gracefully according to the error in the distribution predicted.
	
%Next we show that if the weights are computed according to a distribution over types of impressions, then the error gracefully degrades when the parameters of this distribution are modified. Nodes of one \emph{type} have outgoing edges to the same set of nodes. The theorem below shows that the predictions are a $1-\eps$ approximation when $\opt$ can route almost all of the impressions.

	\begin{theorem}
		%Let $m$ be the number of impressions.
		%For an instance, use $\{p^*_S\}_{S \subseteq V}$ to denote the impression type distribution, where $p_S^*$ represents the proportion of type $S$ impressions in this instance.
		%Given a prediction of this type distribution $\{\predprob_S\}$, we define the prediction error \[\gamma := || \predprob - p^*||_1. \] Employing the prediction $\predprob$, we can obtain a feasible flow whose value is at least
		%\[(1-\epsilon)\opt-2m\gamma,\] where $\opt$ is the maximum flow and $m$ is the number of impressions.

		Let $\{\predprob_S\}_{S \subseteq V}$ be the impression type distribution used to compute the predicted weights. For any constant $\eps> 0$,the predicted weights yield an online flow allocation whose value is at least
		$ (1-\eps)\opt - 2m\gamma. $
		Here $\opt$ is the maximum flow value, $m$ is the number of impressions arriving online, and $\gamma$ is the prediction error.  If $\{p_S^*\}_{S \subseteq V}$ is the actual type distribution in the offline instance, then $\gamma := \|\predprob - p^*\|_1$.

	\end{theorem}
	
	One can interpret the prior theorem as also showing the learnability of the weights when the number of types is small compared to the number of impressions.
It is known that in this case we can efficiently learn the distribution over types via a small sample \cite{Han2015MinimaxEO,pmlr-v40-Kamath15}.
Thus, if we predict the distribution of types and compute the weights using the distribution this will work well when the type proportions are predicted well.
%Thus, in the case of a small number of types, we can observe a small sample of initial arrivals and use them to reliably learn the type distribution and use this learned distribution with the above theorem to get a good performance for these learned weights.

Second, we examine the parameter robustness of the weights and show that the performance degrades linearly in the relative error of the weight parameter.
	
%{\color{red} BEN: we probably need to state state some kind of lower bound for multi layer graphs.}
	
	\begin{theorem}
		
		Consider a prediction of vertex weight $\predw_v$ for each vertex $v\in V$. Due to scale invariance, we can assume that the minimum predicted vertex weight $\predw_{min}=1$.
		Define the prediction error $\eta := \max_{v\in V} (\frac{\predw_v}{\alpha^*_v} ,\frac{\alpha_v^*}{\predw_v} ),$
		where $\{ \alpha_v^* \}_{v\in V}$ are vertex weights that can achieve an $(1-\epsilon)$-approximate solution and $\alpha^*_{min}=1$ for any fixed $\eps >0$.
		Employing predictions $\predw$, we can obtain a solution with competitive ratio
		$ \max(\frac{1}{d+1},\frac{1-\epsilon}{\eta^{2d}}), $
		where $d$ is the diameter of this graph excluding vertex $t$.
		
	\end{theorem}
	
When the prediction error $\eta$ approaches one the performance  smoothly approaches  optimal.	
While the above theorem involves comparing the propagation of the prediction errors in the performance analysis, we also investigate how inaccurate predictions can be adaptively corrected and improved in the 2-layer Adwords case.
For the case of 2-layer DAGs, we give an algorithm that can correct some error in the weights, so that the loss is only logarithmic in the error of the predictions.
% TL: I don't like the next sentence as the result is only interesting for a limited range of eta values
%This way, we show that even if the error is large, we can adapt to the error in the weights.
Moreover, the way we adapt is tight and the best possible up to constant factors.
	
	\begin{theorem}
		
		If the graph $G$ excluding vertex $t$ is bipartite (i.e. $d=2$) and all impressions can be assigned by the optimal solution, given any prediction of vertex weights $\{ \predw_v \}$, we can obtain a solution with competitive ratio
		$\max(\frac{1}{2}, 1-O(\log \eta)).$
		Moreover, this result is tight as no online algorithm with weight predictions can obtain a competitive ratio better than $1-\Omega(\log \eta)$.
		
		
	\end{theorem}
	
	%This is another case where the existence of the weights is useful, since we can use the weights to allocate flow online.


\subsection{Results for Machine Scheduling}



%We give several models to show the weights are efficiently learnable.  We can demonstrate their learnability by establishing that they have low sample complexity.  Additionally, assuming that impressions come from a small number of types, we can show that given a distribution of types and optimal weights for this distribution that if the distribution is changed then the performance degrades proportionally with the change in the distribution.
\noindent \textbf{Paper Organization:} The paper is organized as follows:
Section~\ref{sec:relatedwork} surveys related work.  An overview of our techniques is in Section~\ref{sec:techniques}. The next three sections correspond to the three parts of our results, respectively: the existence of weights, the robustness of weights for online flow allocation, and the learnability of these weights. Missing proofs and additional details are in the Appendix. 

\fi

==> robustnessweight.tex <==
\section{Robustness of Weights}\label{sec:robustnessweight}

In this section, we consider the online flow allocation problem.
The problem is defined on  a Directed-Acyclic-Graph (DAG). In this graph $G(V,E)$, each vertex $v$ in the graph has an associated capacity $c_v$.  
There exists a sink $t$ such that all vertices in the DAG can reach the sink.
%Each node in the last layer is connected to a sink $t$, and thus all nodes in the DAG can reach the sink.

Online source vertices arrive that have no incoming edges (and will never have any incoming edges in the future) and the other layers are offline and fixed.  We will refer to these vertices $I$ as impressions.  When a vertex $i$ arrives, it is connected to a subset of nodes $N_i$.  At the moment of arrival, an algorithm must decide a (fractional) unit flow of $i$ to $t$ that obeys the vertex capacities.  This flow is fixed the moment the vertex arrives.  The goal is to allocate the flows online to maximize the total flow that reaches $t$.

\subsection{Weight predictions}

As we proved in the previous section, for any online instance, there exists a set of vertex weights for $V$ which can return a near optimal solution. Now we predict these vertex weights in the beginning and give an online algorithm based on these weights, which can obtain a competitive ratio related to the error of these predictions.

We first define the prediction error $\eta$.
Consider a prediction of vertex weight $\predw_v$ for each vertex $v\in V$. Due to scale invariance, we can assume that the minimum predicted vertex weight $\predw_{min}=1$. 
Use $\{ \alpha_v^* \}_{v\in V}$ to represent the optimal vertex weights, namely, the weights that can achieve an $(1-\epsilon)$-approximate solution. Similarly, let $\alpha^*_{min}=1$. 

Define the prediction error \[\eta := \max_{v\in V} (\frac{\predw_v}{\alpha^*_v} ,\frac{\alpha_v^*}{\predw_v} ).\]

We have the following claim:


\begin{theorem}\label{thm:weight_predicitive_algorithm}
	Given any weight predictions $\{ \predw \}$, we can obtain a solution with competitive ratio
	\[ \max(\frac{1}{d+1},\frac{1-\epsilon}{\eta^{2d}}), \]
	where $d$ is the diameter of the graph $G$.
\end{theorem}

Due to the reduction in the previous section, w.l.o.g., we can assume that $G$ is $d$-partite in the following.
To prove the theorem above, we first give an online algorithm with competitive ratio $\frac{1-\epsilon}{\eta^{2d}}$, and then show that we can modify this algorithm such that its competitive ratio does not decrease and is always better than $\frac{1}{d+1}$.  

%show that for any online algorithm, we can modify it such that its competitive ratio is always better than $\frac{1}{d+1}$ and then give an online algorithm with competitive ratio $\frac{1-\epsilon}{\eta^{2d}}$.

\begin{lemma}\label{lem:predictive_d_layer}
	If route the flow according to the predicted weights $\{\predw\}$ directly, we can obtain a solution with competitive ratio $(1-\epsilon)/\eta^{2d}$.
\end{lemma}

\begin{proof}
	We give an inductive proof. Consider the first layer $A_1$. For each impression $i$ and $a\in N(i,A_1)$, we have
	\begin{equation}
	\begin{aligned}
	\predx_{i,a} = &\frac{\predw_a}{\sum_{a'\in N(i,A_1)} \predw_{a'} }\\
	\geq& \frac{\alpha_a^*/ \eta}{\sum_{a'\in N(i,A_1)}  \alpha_{a'}^* \eta} \\
	= &  \frac{1}{\eta^2}\frac{\alpha_a^*}{\sum_{a'\in N(i,A_1)}  \alpha_{a'}^*}\\
	= & \frac{1}{\eta^2}x_{i,a}^*
	\end{aligned}
	\end{equation}
	Thus, for each $a\in A_1$, 
	\begin{equation}
	\min(\predA_a, C_a) \geq \frac{1}{\eta^2}\min({Alloc}_a^*, C_a) 
	\end{equation}
	
	Now we prove that if for each vertex $a\in A_j$, \[\min(\predA_a, C_a) \geq \frac{1}{\eta^{2j}}\min({Alloc}_a^*, C_a), \]
	then for each vertex $a\in A_{j+1}$, 
	\[\min(\predA_a, C_a) \geq \frac{1}{\eta^{2(j+1)}}\min({Alloc}_a^*, C_a). \]
	
	For each $a\in A_{j+1}$ and $a'\in N(a,A_j)$, similarly, we have $\predx_{a',a} \geq  \frac{1}{\eta^2}x_{a',a}^*.$ The contribution of vertex $a'$ to $a$ is 
	\begin{equation}
	\min(\predA_{a'},C_{a'}) \predx_{a',a} \geq \frac{1}{\eta^{2(j+1)}}\min({Alloc}_a^*, C_a) x_{a',a}^*.
	\end{equation}
	Thus, for each vertex $a\in A_{j+1}$, 
	\[\min(\predA_a, C_a) \geq \frac{1}{\eta^{2(j+1)}}\min({Alloc}_a^*, C_a). \]
	
	The value $\val$ of our solution is $(1-\epsilon)/\eta^{2d}$-approximated:
	\begin{equation}
	\begin{aligned}
	\val = &\sum_{a\in A_d} \min(\predA_a,C_a ) \\ 
	\geq &\frac{1}{\eta^{2d}}\sum_{a\in A_d} \min(Alloc_a^*,C_a )  \\
	\geq & \frac{1-\epsilon}{\eta^{2d}}\opt. 
	\end{aligned}
	\end{equation}
	
\end{proof}

The above simple algorithm is $(1-\epsilon)$-consistent, but not robust. Now we improve it to obtain both consistency and robustness.
%give another algorithm to obtaining both consistency and robustness.

We say a vertex $v\in V$ is blocked if its capacity is full or all vertices in its neighborhood in the next layer are blocked. Intuitively, if a vertex $v$ is blocked, sending any flow to it cannot increase our objective value. In the previous algorithm, we route each flow according to $\{\predw\}$ directly, indicating we still keep sending arriving flows to some vertices after they are blocked. These flows sent to blocked vertices have no contribution to our objective value. 
%The new algorithm $\algoA'$ deals with such flows in a better way.

%We improve the robustness of our algorithm by deal with 

\begin{algorithm}[t]
	\caption{Online algorithm with weight predictions}
	\label{alg:online_d_layer}
	\KwIn{$G= (I \cup V,E)$ where $I$ arrives online, $\{ C_a \}_{a \in A}$, parameter $\epsilon \in (0,1)$, prediction $\{\predw\}$}
	

	
	\While{an impression $i$ comes }
	{	
		%Initially, set $x_{i,a} = x'_{i,a}=0$ for all $a\in N_i$.
		
		Use $\gamma_i$ to represent the proportion of the feasible flow sent from $i$ to $t$. Initially, $\gamma_i=0$.
		
		\While{ $\gamma_i < 1$ and $i$ can reach $t$ in $G$ }
		{
			Send $(1-\gamma_i)$ flow from $i$ to $t$ according to the predicted weights.
			
			Update $\gamma_i$.
			
			Remove all blocked vertices in $G$.
			
		}
	}
\end{algorithm}

The improved algorithm is stated in Algo~\ref{alg:online_d_layer}. To prove this algorithm has a competitive ratio of $\max(\frac{1}{d+1}, (1-\epsilon)/\eta^{2d})$, we first show that this algorithm always performs better than the previous algorithm, then claim this algorithm always returns a maximal flow and prove that any maximal flow is $\frac{1}{d+1}$-approximated. The definition of a maximal flow will be stated later.

\begin{lemma}\label{lem:improved_online}
	In any instance, Algo~\ref{alg:online_d_layer} performs better than routing the flow according to the predicted weights directly.
\end{lemma}

\begin{proof}
	According to the proportional allocating rules, we have a following claim easily:
	\begin{claim}
		Consider any two neighboring layers $A_j,A_{j+1}$. Under the proportional allocating setting, if for each $a\in A_j$, $\min (Alloc_a,C_a)$ increases, then for each $a\in A_{j+1}$, $\min (Alloc_a,C_a)$ also increases.
	\end{claim}
	
	Recall that for a vertex $a_j$ and $a_{j+1}\in N(a_j,A_{j+1})$, the contribution of $a_j$ to $a_{j+1}$ is $\min (Alloc_{a_j} ,C_{a_j} ) x_{a_j,a_{j+1}} $, where $x_{a_j,a_{j+1}}$ is fixed if the weights is fixed. Since $\min (Alloc_{a_j} ,C_{a_j} )$ increases, its contribution to $a_{j+1}$ also increases. Thus, for each $a\in A_{j+1}$, $\min (Alloc_a,C_a)$ also increases.
	
	The objective value of a solution is the sum of $\min(Alloc_a,C_a)$ over $a\in A_d$. 
	Use $Alloc_a'$ and $Alloc_a$ to represent the value of $Alloc_a$ in Algo~\ref{alg:online_d_layer} and the previous simple algorithm respectively.
	By the claim above, if we prove that for each $a$ in the first layer $A_1$, $\min(Alloc_a',C_a) \geq \min (Alloc_a,C_a)$, this lemma can be proved.
	
	Consider each vertex $a$ in the first layer. If this vertex is blocked in Algo~\ref{alg:online_d_layer}, clearly we have 
	\[ \min(Alloc_a',C_a) \geq C_a \geq \min (Alloc_a,C_a). \]
	If this vertex is not blocked, the new algorithm will not send less flow to it than the old algorithm, thus, we also have
	\[ \min(Alloc_a',C_a) \geq Alloc_a' \geq Alloc_a \geq \min (Alloc_a,C_a), \]
	completing this proof.
\end{proof}

For each impression $i$, use $P_i$ to represent the set of paths from $i$ to the sink $t$, and let $P_i(v) \subseteq P_i$ be the set of paths crossing vertex $v$.
We say a solution is a maximal flow if for any impression $i$ that are not assigned totally, no path in $P_i$ has a free capacity. This definition can be viewed as a generalization of the maximal matching.
According to the statement of Algo~\ref{alg:online_d_layer}, it always returns a maximal flow.
Now we show that any maximal flow is $\frac{1}{d+1}$-approximated.

\begin{lemma}\label{lem:maximal_flow}
	For any maximal flow in $G$, it is $\frac{1}{d+1}$-approximated. 
\end{lemma}

\begin{proof}
	Consider a linear program and dual program of this model.
	%For an impression $i$
	
	\begin{equation}\label{LP}
	\begin{aligned}
	&\max & \sum_{i\in I} \sum_{p\in P_i}& x_{i,p} &\\
	&s.t. &\sum_{p\in P_i} x_{i,p} &\leq 1 \quad &\forall i \in I \\
	&&\sum_{i\in I}\sum_{p\in P_i(v)} x_{i,p} &\leq C_v  & \forall v\in V \\
	&&x_{i,p} &\geq 0 &\forall i\in I,p\in P_i
	\end{aligned}
	\end{equation}
	For each pair $(i,p)$, use variable $x_{i,p}$ to denote the proportion of impression $i$ assigned to path $p$. Using dual variable $\gamma_i$ to represent the constraint that impression $i$ has only one unit and dual variable $y_v$ to represent the capacity constraint of vertex $v$, we can have the following dual program:
	\begin{equation}\label{DP}
	\begin{aligned}
	&\min  &\sum_{v\in V}y_v C_v & +  \sum_{i\in I} \gamma_i &\\
	&s.t. &\sum_{v\in p} y_v + \gamma_i&\geq 1 \quad &\forall i\in I, p\in P_i  \\
	& &y_v,\gamma_i & \geq 0 &\forall i \in I, v\in V
	\end{aligned}
	\end{equation}
	
	Given a maximal solution $\{x_{i,p}\}$ of LP~\eqref{LP}, we now construct a feasible solution of its dual program. Let $\gamma_i$ be the assigned proportion of impression $i$. Namely, \[\gamma_i =\sum_{p\in P_i} x_{i,p}.\] Clearly, we have
	\begin{equation}\label{eq:maximal_1}
	\sum_{i\in I} \sum_{p\in P_i} x_{i,p} = \sum_{i\in I} \gamma_i. 
	\end{equation}
	
	
	Let $y_v$ be the proportion of vertex $v$'s capacity occupied by this solution. Namely,
	\[y_v = (\sum_{i\in I}\sum_{p\in P_i(v)} x_{i,p}) /C_v .\]
	
	Note that the diameter of $G$ is $d$. Any path $p$ crosses at most $d$ vertices in $V$. Thus, if summing over all $y_vC_v$, each $x_{i,p}$ is counted at most $d$ times. Thus, we have
	\begin{equation}\label{eq:maximal_2}
	d\sum_{p\in P_i} x_{i,p} \geq \sum_{v\in V}y_v C_v. 
	\end{equation}
	
	Combining Eq~\eqref{eq:maximal_1} and Eq~\eqref{eq:maximal_2}, we have
	\begin{equation}
	(d+1)\sum_{p\in P_i} x_{i,p} \geq \sum_{v\in V}y_v C_v + \sum_{i\in I} \gamma_i.
	\end{equation}
	
	If $\{y_v,\gamma_i  \}$ is feasible, then the maximal flow is $\frac{1}{d+1}$-approximated. For any pair $(i,p)$, if $\gamma_i=1$, its constraint is satisfied. Otherwise, according to our algorithm, path $p$ has no free capacity, indicating that there exists a vertex $v$ in this path with $y_v=1$. So we still have $ \sum_{v\in p} y_v + \gamma_i\geq 1.$ Thus, $\{y_v,\gamma_i  \}$ is feasible and this maximal flow is $\frac{1}{d+1}$-approximated.
	
	
\end{proof}

Combing Lemma~\ref{lem:predictive_d_layer}, Lemma~\ref{lem:improved_online} and Lemma~\ref{lem:maximal_flow}, Theorem~\ref{thm:weight_predicitive_algorithm} can be proved directly.





\subsection{A special case that $d=1$}

\begin{algorithm}[t]
	\caption{Online algorithm with predictions when $d=1$}
	\label{alg:online}
	\KwIn{$G= (I \cup A\cup \{t\},E)$ where $I$ and $E$ arrive online, $\{ C_a \}_{a \in A}$, parameter $\epsilon \in (0,1)$, prediction $\{\predw\}$}
	Create a same imaginary instance as the input instance, we use $x'$ and $Alloc'$ to denote the assignment in this instance. \
	
	\While{an impression $i$ comes }
	{	
		Initially, set $x_{i,a} = x'_{i,a}=0$ for all $a\in N_i$.
		
		
		\While{$\sum_{a\in N_i}x_{i,a}<1$}
		{
			For each $a\in N_i$, increase $x_{i,a}$ and $x'_{i,a}$ with rate $\frac{\predw_a}{\sum_{a' \in N_i} \predw_{a'} }$ until $\sum_{a\in N_i}x_{i,a}=1$ or there exists one advertiser $a$ such that $Alloc'_a = (1+\epsilon)^2C_a$.
			
			\While{there exists one advertiser $a$ such that $Alloc'_a \geq (1+\epsilon)^2C_a$}
			{
				For each $a \in A$, if $Alloc_a' \geq (1+\epsilon)^2C_a$, $\predw_a \leftarrow \predw_a / (1+\epsilon)$.\
				
				Update each $x_{i,a}'$ and $Alloc_a'$ according to new $\{ \predw_a\}$.			
			}		
		}
	}
\end{algorithm}

If $d=1$, this problem is an online bipartite matching problem. In this special case, we show that we can come up with an algorithm with a better competitive ratio:

\begin{theorem}\label{thm:online_algo}
	Assuming that all impressions can be assigned and all advertisers can be filled out, for any given $\epsilon\in (0,1)$, Algo~\ref{alg:online} can obtain a competitive ratio of
	\[ 1-4\epsilon\log_{(1+\epsilon)} \eta-3\epsilon. \]
\end{theorem}

%\begin{proof}[\textbf{Proof of Theorem~\ref{thm:online_algo}}]
We first prove that our algorithm can terminate. Namely, when a new impression arrives, we can always find the weights $\{ \predw \}$ such that in the imaginary instance, $\forall a\in A$, $Alloc_a' < (1+\epsilon)^2C_a$.

%Since we assume that all impressions can be assigned by a set of optimal weights $\{ \alpha^*\}$, $\forall a\in A$, 
Let $\{ \alpha^*\}$ be the optimal weights. Since we assume that all impressions can be assigned, we can assume that for any advertiser $a$, we have $Alloc_a^* < (1+\epsilon)C_a$. We give the following claim to show that the algorithm will not fall into an endless loop:
\begin{claim}\label{claim:terminate}
	In any time during the algorithm, for any $a\in A$, $\predw_a \geq \alpha_a^*/\eta$.
\end{claim}
\begin{proof}
	Assuming that at some point, there existed some  $\predw_a < \alpha_a^*/\eta$.
	Use $b$ to represent a such vertex.
 	Consider the first time $t$ that this event occurred. 
	Clearly, $Alloc_{b}'(t-1) \geq (1+\epsilon)^2C_{b}$. Since $t$ is the first time, we also have for any $a$, $\predw_{a}(t-1) \geq \alpha_{a}^* /\eta$ and $\predw_{b}(t-1) < \alpha_{b}^*(1+\epsilon) /\eta$. For any $x'_{i,b}$ in time $t-1$, we have that
	\begin{equation}
	x'_{i,b}(t-1) = \frac{\predw_{b}(t-1)}{\sum_{a\in N_i} \predw_a(t-1)} < \frac{(1+\epsilon) \alpha_{b}^*/\eta }{\sum_{a\in N_i} \alpha_a^*/\eta  }  = (1+\epsilon) x_{i,b}^*.
	\end{equation}
	Thus, we know in the time $t-1$, 
	\begin{equation}
	Alloc_{b}'(t-1) < (1+\epsilon) Alloc_{b}^* < (1+\epsilon)^2C_{b},
	\end{equation}
	contradicting to the fact that $Alloc_{b}'(t-1) \geq (1+\epsilon)^2C_{b}$. 
\end{proof}

According to Claim~\ref{claim:terminate}, we can make sure that our algorithm can terminate because we can not keep decreasing $\predw$. The value of ${\predw}$ will stop when it is close to the nearest ${\alpha^*/\eta}$.

For any advertiser $a$, use $k$ to represent the number of times that its weight decreased and $w_1,w_2,...,w_k$ to denote $k$ different values of its weight. Our initial prediction $\predw_a$ is viewed as $w_0$. Since each time, the weight decreased by $(1+\epsilon)$, we have $w_k = w_0/(1+\epsilon)^k$.
Due to Claim~\ref{claim:terminate}, $w_k \geq \beta_a^*$. Thus, 
\begin{equation}
\begin{aligned}
\frac{w_0}{(1+\epsilon)^k}& \geq \alpha_a^*/\eta \\
(1+\epsilon)^k &\leq \eta \frac{\predw_a}{\alpha_a^*} \\
k \leq 2\log&_{(1+\epsilon)} \eta
\end{aligned}
\end{equation}
Namely, the weight decreased at most $2\log_{(1+\epsilon)} \eta$ times.
Use $Alloc_a^{(j)}$ to represent the number of impressions that assigned to $a$ when $a$'s weight is $w_j$. In the following, we will try to bound each $Alloc_a^{(j)}$ to give a upper bound of the final $Alloc_a$.

\begin{lemma}~\label{lem:before_decrease}
	For any advertiser $a$, $Alloc_a^{(0)} \leq (1+\epsilon)^2 C_a$.
\end{lemma}

\begin{proof}
	This lemma can be proved very easily. For any advertiser $a$, if its weight has not decreased so far, we have $Alloc_a' < (1+\epsilon)^2C_a$.
	
	
	When one impression arrived, in the first step, the increments of $Alloc_a$ and $Alloc_a'$ are the same. In the second step, $Alloc_a'$ may change due to the decrease of other weights. Since $\predw_a$ has not decreased, $Alloc_a'$ cannot decrease in this step. Thus, we have $Alloc_a \leq Alloc_a' < (1+\epsilon)^2C_a$.
\end{proof}


\begin{lemma}~\label{lem:after_decrease}
	For any advertiser $a$ and any $j \geq 1$, $Alloc_a^{(j)} \leq 2\epsilon C_a$.
\end{lemma}

\begin{proof}
	As we mentioned above, if $\predw_a$ did not change, the increment of $Alloc_a$ is no more than the increment of $Alloc_a'$. Thus, if we prove that during the period that $\predw_a = w_j$, $Alloc_a'$ increased at most $3\epsilon C_a$, this lemma can be proved.
	
	Consider the moment that advertiser $a$'s weight decreased from $w_{j-1}$ to $w_j$. Use $Alloc_a'(-)$ and $Alloc_a'(+)$ to denote the allocation in the imaginary instance before and after this decrease. Clearly, we have $Alloc_a'(-)\geq (1+\epsilon)^2C_a$. When the weight decreased by $(1+\epsilon)$, the allocation decreased by at most $(1+\epsilon)$. So after this decrease, 
	\[ Alloc_a'(+) \geq Alloc_a'(-)/(1+\epsilon) \geq (1+\epsilon)C_a. \]
	
	During the period that $\predw_a = w_j$, $Alloc_a'$ cannot become larger than $(1+\epsilon)^2C_a$ according to our algorithm. Thus, the increment of $Alloc_a'$ in this period is at most 
	\[ (1+\epsilon)^2C_a - (1+\epsilon)C_a\leq 2\epsilon C_a, \]
	
	completing this proof.
	
\end{proof}

Combining Lemma~\ref{lem:before_decrease} and Lemma~\ref{lem:after_decrease}, we have 
\begin{equation}
Alloc_a = \sum_{j} Alloc_a^{(j)} \leq (1+3\epsilon+4\epsilon \log_{(1+\epsilon)}\eta)C_a
\end{equation}

This equation indicates that for each advertiser $a$, there are at most $(3\epsilon+4\epsilon \log_{(1+\epsilon)}\eta) C_a$ impressions having no contribution to the objective value. Assuming that all advertisers can be filled out, we have 

\begin{equation}
\begin{aligned}
\sum_a \min(Alloc_a,C_a) & \geq \sum_a C_a - \sum_a (3\epsilon+4\epsilon \log_{(1+\epsilon)}\eta) C_a \\
& \geq OPT(1-4\epsilon \log_{(1+\epsilon)} \eta -3\epsilon)
\end{aligned}
\end{equation}

the proof of Theorem~\ref{thm:online_algo} has been completed. 
And similarly with Algo~\ref{alg:online_d_layer}, we can also come up with an algorithm with a competitive ratio of $\max(1-4\epsilon\log_{(1+\epsilon)} \eta-3\epsilon, 1/2)$. When the predictions are correct, we can obtain a near optimal solution. When $\eta$ is large, the ratio will not become worse than $1/2$.

In the next subsection, we show this competitive ratio is near optimal.


\subsection{Upper bound }

In this subsection, we provide an upper bound against online predictive matching algorithms:

\begin{theorem}\label{thm:bound}
	For any online algorithm with weight predictions, even if $d=1$, its competitive ratio is not better than $1-O(\log\eta)$.
\end{theorem}

This bound indicates that our algorithm is near optimal. The basic idea is to construct a distribution of inputs and predictions such that $\eta$ is very small and the expectation of any algorithm's competitive ratio is at most $1-\log \eta$, indicating the worst ratio among these instances cannot be better than this expectation value.  

More specifically, the graph $G$ has $n$ advertisers $(a_1,...,a_n)$ and $n$ impressions $(i_1,...,i_n)$. Sample a uniform random permutation $\pi$ of set $[n]$. Given any parameter $0< s < n$, define the edge set to be
\[ \E = \{ (a_{\pi(j)}, i_k)  | j,k \leq s  \} \cup \{ (a_{\pi(j)}, i_k) | j >s \text{ and } 1\leq k \leq n \}. \]
Note that this parameter $s$ will be served as an bridge between the competitive ratio and the prediction error.

The impressions arrive in the order $i_1,i_2,...,i_n$. For each advertiser $a$, we set its capacity $C_a$ to be $1$ and its predictive weight $\predw_a$ to be $1$.

We can see Fig~\ref{fig:upperbound} as an illustration. Given the parameter $s$, we can partition all advertisers into two sets according to the permutation $\pi$. The first $s$ impressions are adjacent to all advertisers, while the last $n-s$ impressions only connect to all purple advertisers.

\begin{figure}[t]\label{fig:upperbound}
	\centering
	\includegraphics[width=0.6\linewidth]{Figures/upper_bound_instance}
	\caption{An illustration of the constructed instance. }
\end{figure}

We first give the expected competitive ratio of this instance, then analyze $\{ \beta^* \}$ and give $\eta$. As mentioned above, both the ratio and $\eta$ will be related to parameter $s$. Thus, we draw the conclusion that if $s$ satisfies some conditions, the ratio will be at most $1-\log \eta$.

\begin{lemma}\label{lem:bound_ratio}
	Let $p$ be $\frac{n-s}{n}$,  the expected competitive ratio $r$ of any online algorithm is at most $1-p(1-p)$.
\end{lemma}
\begin{proof}
	Clearly, for any permutation $\pi$, there is always a perfect matching in this graph. Namely, the expected optimal value $\opt$ is $n$. Consider the expected value of each $x_{a_{\pi(j)},i_k}$. When $1\leq k\leq s$, this value is at most $\frac{1}{n}$ because for any two advertisers $a_{\pi(j_1)}$ and $a_{\pi(j_2)}$, we have $E(x_{a_{\pi(j_1)},i_k}) = E(x_{a_{\pi(j_2)},i_k})$ by symmetry, and the sum of all advertisers' values is at most $1$. Similarly, when $s<k<n$, $x_{a_{\pi(j)},i_k}$ is $0$ if $j \leq s$ and at most $\frac{1}{n-s}$ if $j>s$. Thus, each green advertiser matches at most $s/n$ impressions while each purple advertiser matches at most $1$ impressions. The expected competitive ratio of any online fractional matching algorithm can be bounded:
	
	\begin{equation}
	\begin{aligned}
	r &= \frac{\sum_{j=1}^{n} \sum_{k=1}^{n}E(x_{a_{\pi(j),i_k}}) }{n}  \\
	&\leq \frac{1}{n}(\frac{s}{n}\cdot s + n-s)\\
	& = 1-\frac{(n-s)s}{n^2} \\
	& = 1- p(1-p)
	\end{aligned}
	\end{equation}
\end{proof}

\begin{lemma}\label{lem:bound_error}
	Given any permutation $\pi$ and any $\epsilon \in (0,1)$, there exists a set of weights $\{ \beta^* \}$ with $\eta_{\beta^*} = p/\epsilon$ such that it can achieve a $(1-\epsilon)$-approximated fractional matching.  
\end{lemma}

\begin{proof}
	Since the first $s$ advertisers in the permutation are equivalent, we let $\beta^*_{a_{\pi(1)}} = \beta^*_{a_{\pi(2)}} = ... = \beta^*_{a_{\pi(s)}} = w_1.$ Similarly, we have $\beta^*_{a_{\pi(s+1)}} = \beta^*_{a_{\pi(s+2)}} = ... = \beta^*_{a_{\pi(n)}}=w_2.$ Clearly, the last $n-s$ impressions will fill out the last $n-s$ advertisers. For each one in the first $s$ impressions, the unmatched proportion is the proportion that assigned to the last $n-s$ advertisers. Letting $w_2=1$, this proportion is $\frac{(n-s)}{sw_1+(n-s)}$. Thus, we can compute the size of the fractional matching obtained by these weights:
	\begin{equation}
	\begin{aligned}
	\val = n- \frac{s(n-s)}{sw_1+(n-s)}
	\end{aligned}
	\end{equation}
	We desire that these weights can obtain a $(1-\epsilon)$-approximated fractional matching. Thus, we have
	\begin{equation}
	\begin{aligned}
	n- \frac{s(n-s)}{sw_1+(n-s)} \geq (1-\epsilon)n 
	\end{aligned}
	\end{equation}
	Solving the inequality above, we have
	\begin{equation}
	\begin{aligned}
	w_1 \geq \frac{p}{\epsilon} -\frac{p}{1-p}
	\end{aligned}
	\end{equation}
	If $w_1=\frac{p}{\epsilon}$, we can achieve a $(1-\epsilon)$-approximated fractional matching. Since all predicted weights equal one, when $p > \epsilon$, the error is $p/\epsilon$, completing the proof.
\end{proof}

According to Lemma~\ref{lem:bound_error} and the definition of $\eta$, we have $\eta \leq p/\epsilon$. When $0<\log (\frac{p}{\epsilon}) \leq p(1-p)$, we can bounded the expected competitive ratio:
\begin{equation}
r \leq 1-p(1-p) \leq 1-\log (\frac{p}{\epsilon})  \leq 1- \log \eta,
\end{equation}
completing the proof of Theorem~\ref{thm:bound}.

\subsection{Distribution predictions}

Consider a DAG $G(V,E)$. For any subset $S\subseteq V$, we say the type of a impression $i$ is $S$ if its neighborhood is $S$. 
For an instance, use $\{p^*_S\}$ to denote the impression type distribution, where $p_S^*$ represents the proportion of impressions with type $S$ in this instance.

Intuitively, under some random settings, the impression type distributions of different online instance are close to each other. 
In the subsection, we give a prediction of this impression type distribution $\{\predprob_S\}$ and define the prediction error:
\[\gamma := || \predprob - p^*||_1. \]

Given a predicted distribution $\{\predprob_S\}$, we can compute a set of optimal weights $\{\predw_v\}$ for it.
We show that if use these weights $\{\predw_v\}$ directly on an instance with distribution $\{p^*_S\}$, our competitive ratio can be bounded by a function of the prediction error.

\begin{theorem}\label{thm:type_model}
	Routing flow directly according to $\{\predw_v\}$ returns a feasible flow whose value is at least
	\[(1-\epsilon)\opt-2m\gamma,\] where $\opt$ is the maximum flow and $m$ is the number of impressions.
\end{theorem}

\begin{proof}
	Use $\predI$ and $I^*$ to represent the impression set with distribution $\{ \predprob_S \}$ and $\{ p^*_S \}$ respectively.
	The weights $\{ \predw_v \}$ are the optimal weights of the instance $(\predI,G)$. 
	Add a source $s$ into the instance $(\predI,G)$, which is adjacent to each $i\in \predI$. 
	The new graph is denoted by $\predG$.
	According to the reduction, w.l.o.g., we can assume $\predG$ is an $(s$-$t)$ $d$-partite graph.
	Use $\val(\predw,\predG)$ to represent the value of flow if routing according to $\{\predw_v\}$ on graph $\predG$.
	Similarly, we can define $G^*$ and $\val(\predw,G^*)$.
	Note that for any impression set, we can shrink the impression $i$ with the same type into one vertex. Thus, $\predG$ and $G^*$ can be viewed as a same graph with different capacity functions on the impression layer $I$.
	
	
	Our goal is to prove that 
	\begin{equation}\label{eq:type_model}
	\val(\predw,G^*) \geq (1-\epsilon)\opt-2m\gamma. 
	\end{equation}
	
	
	
	As shown above, in graph $\predG$, there exists an $s$-$t$ cut $\C$ such that 
	\begin{equation}\label{eq:type_eq_main}
	\val(\predw,\predG) \geq (1-\epsilon) C(\C,\predG),
	\end{equation}
	where $C(\C,\predG)$ is the value of cut $\C$ based on the capacity function of $\predG$.
	
	The basic framework of proving Theorem~\ref{thm:type_model} is first showing that the performances of $\{\predw\}$ is close in $\predG$ and $G^*$:
	\begin{equation}\label{eq:type_eq_1}
	\val(\predw,G^*) \geq \val(\predw,\predG) - m\gamma,
	\end{equation}
	and then proving the values of cut $\C$ in $\predG$ and $G^*$ is also close:
	\begin{equation}\label{eq:type_eq_2}
	C(\C,\predG)\geq C(\C,G^*) - m\gamma.
	\end{equation}
	
	Since $ C(\C,G^*)$ is the upper bound of $\opt$, Eq~\eqref{eq:type_model} can be proved directly by combining Eq~\eqref{eq:type_eq_main}, Eq~\eqref{eq:type_eq_1} and Eq~\eqref{eq:type_eq_2}.
	
	Create a new graph $G'$ based on $G^*$ and $\predG$, where the only difference is the capacity function of impression layer $I$. For each impression type $S$, its capacity in $G'$ is the minimum value of its capacity in $G^*$ and $\predG$:
	\[ C(S, G' ) = \min (C(S,G^*),C(S,\predG)  ). \]
	Thus, 
	\[ |C(S,G')-C(S,\predG) | \leq m|p^*_S - \predprob_S|, \]
	indicating that with the same weights, if increase the capacity of impression type $S$ from $C(S,G')$ to $C(S,\predG)$, the objective value increases at most $m|p^*_S - \predprob_S|$. So we have
	\[ |\val(\predw,G')-\val(\predw,\predG)| \leq m\sum_S |p^*_S - \predprob_S | \leq m\gamma  \]
	
	Since the capacity of each vertex in $G^*$ is no less than that in $G'$, we have 
	\[ \val(\predw,G^*) \geq \val(\predw,G'). \]
	Thus,
	\[ \val(\predw,G^*) \geq \val(\predw,\predG) - m \gamma. \]
	
	Eq~\eqref{eq:type_eq_2} can also be proved in the same way:
	\[ C(\C,\predG) \geq C(\C,G') \geq C(\C,G^*) - m\gamma,\]
	completing the proof of Eq~\eqref{eq:type_eq_main}.
\end{proof}






